Non-Euclidean Spatial Graph Neural Network

Spatial networks are networks whose graph topology is constrained by their embedded spatial space. Understanding the coupled spatial-graph properties is crucial for extracting powerful representations from spatial networks. Therefore, merely combining individual spatial and network representations cannot reveal the underlying interaction mechanism of spatial networks. Besides, existing spatial network representation learning methods can only consider networks embedded in Euclidean space, and can not well exploit the rich geometric information carried by irregular and non-uniform non-Euclidean space. In order to address this issue, in this paper we propose a novel generic framework to learn the representation of spatial networks that are embedded in non-Euclidean manifold space. Specifically, a novel message-passing-based neural network is proposed to combine graph topology and spatial geometry, where spatial geometry is extracted as messages on the edges. We theoretically guarantee that the learned representations are provably invariant to important symmetries such as rotation or translation, and simultaneously maintain sufficient ability in distinguishing different geometric structures. The strength of our proposed method is demonstrated through extensive experiments on both synthetic and real-world datasets.

==> recycle.tex <==
\begin{tabular}{c|ccccccccc}
\hline
Target & GCN  & GIN        & PointNet   & PPFNet     & MeshCNN    & CurvaNet   & SchNet     & SGMP       & Ours       \\ \hline
$r_c$ & 3.35 & 2.55 & 3.45 & 2.68 & 2.06 & 1.54 & 0.97 & 1.08 & 0.83 \\
$D$   & 2.20 & 2.73 & 2.62 & 1.98 & 1.87 & 1.93 & 1.94 & 1.86 & 1.67 \\
$r$   & 2.63 & 2.60 & 1.95 & 2.07 & 1.60 & 1.74 & 1.98 & 1.88 & 1.47 \\ \hline
\end{tabular}

\begin{table}[]
\begin{tabular}{llllllllll}
          & GCN         & GIN         & PointNet    & PPFNet      & MeshCNN     & CurvaNet    & SchNet      & SGMP        & Ours        \\
HCP       & 0.835$\pm$0.014 & 0.920$\pm$0.007 & 0.645$\pm$0.027 & 0.927$\pm$0.004 & 0.684$\pm$0.021 & 0.559$\pm$0.025 & 0.876$\pm$0.008 & 0.896$\pm$0.012 & 0.943$\pm$0.005 \\
Flight-NA & 0.674$\pm$0.015 & 0.706$\pm$0.006 & 0.694$\pm$0.011 & 0.720$\pm$0.004 & 0.521$\pm$0.023 & 0.597$\pm$0.019 & 0.710$\pm$0.008 & 0.698$\pm$0.004 & 0.731$\pm$0.005 \\
Flight-GL & 0.722$\pm$0.003 & 0.746$\pm$0.014 & 0.737$\pm$0.010 & 0.759$\pm$0.009 & 0.556$\pm$0.032 & 0.628$\pm$0.025 & 0.750$\pm$0.008 & 0.715$\pm$0.012 & 0.782$\pm$0.005 \\
SHREC     & 0.525$\pm$0.042 & 0.533$\pm$0.034 & 0.567$\pm$0.007 & 0.887$\pm$0.010 & 0.910$\pm$0.003 & 0.902$\pm$0.004 & 0.575$\pm$0.012 & 0.896$\pm$0.005 & 0.918$\pm$0.004 \\
FAUST     & 0.535$\pm$0.010 & 0.783$\pm$0.013 & 0.905$\pm$0.010 & 0.918$\pm$0.005 & 0.903$\pm$0.008 & 0.923$\pm$0.004 & 0.865$\pm$0.023 & 0.840$\pm$0.035 & 0.928$\pm$0.005
\end{tabular}
\end{table}
